Adversarially Robust CLIP Models Can Induce Better (Robust) Perceptual Metrics

Measuring perceptual similarity is a key tool in computer vision. In recent years perceptual metrics based on features extracted from neural networks with large and diverse training sets, e.g. CLIP, have become popular. At the same time, the metrics extracted from features of neural networks are not adversarially robust. In this paper we show that adversarially robust CLIP models, called R-CLIP$_\textrm{F}$, obtained by unsupervised adversarial fine-tuning induce a better and adversarially robust perceptual metric that outperforms existing metrics in a zero-shot setting, and further matches the performance of state-of-the-art metrics while being robust after fine-tuning. Moreover, our perceptual metric achieves strong performance on related tasks such as robust image-to-image retrieval, which becomes especially relevant when applied to "Not Safe for Work" (NSFW) content detection and dataset filtering. While standard perceptual metrics can be easily attacked by a small perturbation completely degrading NSFW detection, our robust perceptual metric maintains high accuracy under an attack while having similar performance for unperturbed images. Finally, perceptual metrics induced by robust CLIP models have higher interpretability: feature inversion can show which images are considered similar, while text inversion can find what images are associated to a given prompt. This also allows us to visualize the very rich visual concepts learned by a CLIP model, including memorized persons, paintings and complex queries.

==> figures/text-inversion-adam-1.tex <==
\begin{figure*}[]
\centering
%\tiny
\footnotesize
% Row 1
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Mona Lisa by Leonardo da Vinci
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Guernica by\\Pablo Picasso
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        The Last Supper by Leonardo da Vinci
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        The Scream by Edvard Munch
    \end{minipage}%    
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Isaac Newton
    \end{minipage}% 
\end{minipage}


\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_12-10-47-target=Mona_Lisa_by_Leonardo_da_Vinci-batch1-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_12-35-50-target=Guernica_by_Pablo_Picasso-batch1-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_13-15-46-target=The_Last_Supper_by_Leonardo_da_Vinci-batch4-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_13-30-53-target=The_Scream_by_Edvard_Munch-batch2-img0-adv.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_14-00-51-target=Isaac_Newton-batch3-img0-adv.png}
    \end{subfigure}% 
\end{minipage}

% row 2
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{1mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Yoshua Bengio
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Boris Johnson
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Elon Musk
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        The Terminator
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        An alien marketplace
    \end{minipage}%
\end{minipage}

\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_14-20-57-target=Yoshua_Bengio-batch2-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_14-45-59-target=Boris_Johnson-batch2-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_15-15-55-target=Elon_Musk-batch3-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_15-26-04-target=The_Terminator-batch0-img0-adv.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_15-56-08-target=An_alien_marketplace-batch1-img0-adv.png}
    \end{subfigure}%
\end{minipage}

% Row 3
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{1mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        An octopus\\playing chess
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A penguin at\\the beach
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A dragon playing\\the piano
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A squirrel riding\\a skateboard
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A werewolf howling\\at a full moon
    \end{minipage}%    
\end{minipage}

\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_16-16-10-target=An_octopus_playing_chess-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_16-46-15-target=A_Penguin_at_the_beach-batch1-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_17-16-15-target=A_dragon_playing_the_piano-batch2-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_17-46-15-target=A_squirrel_riding_a_skateboard-batch3-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-14_18-16-15-target=A_werewolf_howling_at_a_full_moon-batch4-img0-adv.png}
    \end{subfigure}%  
\end{minipage}

\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{1mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Louvre Museum
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Great Wall of China
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        White House
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Marie Curie
    \end{minipage}%    
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Rosa Parks
    \end{minipage}% 
\end{minipage}


\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-23_23-14-30-target=Louvre_Museum-batch4-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-23_23-24-38-target=Great_Wall_of_China-batch1-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-23_23-54-43-target=White_House-batch2-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_00-24-59-target=Marie_Curie-batch3-img0-adv.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_00-55-06-target=Rosa_Parks-batch4-img0-adv.png}
    \end{subfigure}% 
\end{minipage}

\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{1mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Margaret Thatcher
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Angela Merkel
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Cleopatra
    \end{minipage}%
    \begin{minipage}[t]{0.165\textwidth}
        \centering
        Joan of Arc
    \end{minipage}%
    \begin{minipage}[t]{0.215\textwidth}
        \centering
        \spaceskip=0.75\fontdimen2\font plus 0.75\fontdimen3\font minus 0.75\fontdimen4\font   % reduce word spacing
        \mbox{An astronaut riding a horse}
    \end{minipage}%
\end{minipage}

\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_01-15-14-target=Margaret_Thatcher-batch3-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_01-40-22-target=Angela_Merkel-batch3-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_01-50-32-target=Cleopatra-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_02-20-40-target=Joan_of_Arc-batch1-img0-adv.png}
    \end{subfigure}% 
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_02-40-49-target=An_astronaut_riding_a_horse-batch0-img0-adv.png}
    \end{subfigure}%
\end{minipage}


\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{1mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A dragon\\playing chess
    \end{minipage}%
    \begin{minipage}[t]{0.175\textwidth}
        \centering
        A robot cooking\\a meal
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering 
        A detective solving a mys-\\tery in a haunted house
    \end{minipage}%
    \begin{minipage}[t]{0.175\textwidth}
        \centering
        An alien visiting\\a museum
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A scientist discovering\\a new planet
    \end{minipage}%    
\end{minipage}

\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_03-10-52-target=A_dragon_playing_chess-batch1-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_03-40-58-target=A_robot_cooking_a_meal-batch2-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_04-01-06-target=A_detective_solving_a_mystery_in_a_haunted_house-batch1-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_04-41-11-target=An_alien_visiting_a_museum-batch4-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/adam/2024-03-24_04-56-21-target=A_scientist_discovering_a_new_planet-batch2-img0-adv.png}
    \end{subfigure}%  
\end{minipage}

\caption{\textbf{Text inversion variant.} \chs{update} The text inversions in this figure are created using an augmentation procedure in the optimization process as described in \cref{app:text-inv-alternative}.}
\label{fig:text-inv-adam1}
\end{figure*}

==> figures/text-inversion-app-workshop.tex <==
\begin{figure*}[h]
\centering
%\tiny
\footnotesize
% Row 1
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Louvre Museum
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Great Wall of China
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        White House
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Marie Curie
    \end{minipage}%    
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Rosa Parks
    \end{minipage}% 
\end{minipage}


% eps=100, initial_stepsize=10
\vspace{0.5ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-16-03-target=Louvre_Museum-batch0-img9-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-10-31-target=Great_Wall_of_China-batch0-img4-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-17-07-target=White_House-batch0-img4-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-00-48-target=Marie_Curie-batch0-img8-adv.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-01-22-target=Rosa_Parks-batch0-img4-adv.png}
    \end{subfigure}% 
\end{minipage}

\vspace{0.5ex}
% row 2
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-58-02-target=Louvre_Museum-batch0-img5-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-55-08-target=Great_Wall_of_China-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-59-08-target=White_House-batch0-img5-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-45-15-target=Marie_Curie-batch0-img7-adv.png}
    \end{subfigure}% 
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-45-47-target=Rosa_Parks-batch0-img0-adv.png}
    \end{subfigure}%
\end{minipage}

% row 3  
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{2mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Margaret Thatcher
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Angela Merkel
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Cleopatra
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Joan of Arc
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        An astronaut riding\\a horse
    \end{minipage}%
\end{minipage}

\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-01-56-target=Margaret_Thatcher-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-04-44-target=Angela_Merkel-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-05-15-target=Cleopatra-batch0-img9-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-05-49-target=Joan_of_Arc-batch0-img1-adv.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-19-16-target=An_astronaut_riding_a_horse-batch0-img2-adv.png}
    \end{subfigure}%
\end{minipage}

%  eps=200, initial_stepsize=none (i.e. 400)
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-46-20-target=Margaret_Thatcher-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-49-04-target=Angela_Merkel-batch0-img8-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-49-37-target=Cleopatra-batch0-img5-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-50-11-target=Joan_of_Arc-batch0-img2-adv.png}
    \end{subfigure}% 
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-01-20-target=An_astronaut_riding_a_horse-batch0-img2-adv.png}
    \end{subfigure}%
\end{minipage}


% Row 5  
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{2mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A dragon\\playing chess
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A robot cooking\\a meal
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A detective solving a\\mystery in a haunted house
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        An alien visiting\\a museum
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A scientist discovering\\a new planet
    \end{minipage}%    
\end{minipage}

% Row 6  eps=200, initial_stepsize=none (i.e. 400)
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-20-52-target=A_dragon_playing_chess-batch0-img7-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-20-21-target=A_robot_cooking_a_meal-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-23-03-target=A_detective_solving_a_mystery_in_a_haunted_house-batch0-img7-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-22-30-target=An_alien_visiting_a_museum-batch0-img6-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-25-12-target=A_scientist_discovering_a_new_planet-batch0-img7-adv.png}
    \end{subfigure}%  
\end{minipage}

% Row 7


\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-02-58-target=A_dragon_playing_chess-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-02-26-target=A_robot_cooking_a_meal-batch0-img9-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-05-08-target=A_detective_solving_a_mystery_in_a_haunted_house-batch0-img7-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-04-35-target=An_alien_visiting_a_museum-batch0-img2-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-07-09-target=A_scientist_discovering_a_new_planet-batch0-img0-adv.png}
    \end{subfigure}%  
\end{minipage}

% \vspace{1em}
\caption{\textbf{Text inversion.} We show additional text inversion examples for \rclip. Small initial step-size and large initial step-size are considered in the first and second rows respectively.
}
\label{fig:text-inv-app}
\end{figure*}

==> figures/text-inversion-app.tex <==
\begin{figure*}[]
\centering
\tiny
% Row 1
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\textwidth}
    \vspace{0pt}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Louvre Museum
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Great Wall of China
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        White House
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Marie Curie
    \end{minipage}%    
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Rosa Parks
    \end{minipage}% 
\end{minipage}


% eps=100, initial_stepsize=10
\vspace{0.5ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\textwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-16-03-target=Louvre_Museum-batch0-img9-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-10-31-target=Great_Wall_of_China-batch0-img4-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-17-07-target=White_House-batch0-img4-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-00-48-target=Marie_Curie-batch0-img8-adv.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-01-22-target=Rosa_Parks-batch0-img4-adv.png}
    \end{subfigure}% 
\end{minipage}

\vspace{0.5ex}
% row 2
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\textwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-58-02-target=Louvre_Museum-batch0-img5-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-55-08-target=Great_Wall_of_China-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-59-08-target=White_House-batch0-img5-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-45-15-target=Marie_Curie-batch0-img7-adv.png}
    \end{subfigure}% 
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-45-47-target=Rosa_Parks-batch0-img0-adv.png}
    \end{subfigure}%
\end{minipage}

% row 3  
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\textwidth}
    \vspace{2mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Margaret Thatcher
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Angela Merkel
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Cleopatra
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Joan of Arc
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        An astronaut riding\\a horse
    \end{minipage}%
\end{minipage}

\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\textwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-01-56-target=Margaret_Thatcher-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-04-44-target=Angela_Merkel-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-05-15-target=Cleopatra-batch0-img9-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-05-49-target=Joan_of_Arc-batch0-img1-adv.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-19-16-target=An_astronaut_riding_a_horse-batch0-img2-adv.png}
    \end{subfigure}%
\end{minipage}

%  eps=200, initial_stepsize=none (i.e. 400)
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\textwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-46-20-target=Margaret_Thatcher-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-49-04-target=Angela_Merkel-batch0-img8-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-49-37-target=Cleopatra-batch0-img5-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_13-50-11-target=Joan_of_Arc-batch0-img2-adv.png}
    \end{subfigure}% 
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-01-20-target=An_astronaut_riding_a_horse-batch0-img2-adv.png}
    \end{subfigure}%
\end{minipage}


% Row 5  
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\textwidth}
    \vspace{2mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A dragon\\playing chess
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A robot cooking\\a meal
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A detective solving a\\mystery in a haunted house
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        An alien visiting\\a museum
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A scientist discovering\\a new planet
    \end{minipage}%    
\end{minipage}

% Row 6  eps=200, initial_stepsize=none (i.e. 400)
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\textwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-20-52-target=A_dragon_playing_chess-batch0-img7-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-20-21-target=A_robot_cooking_a_meal-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-23-03-target=A_detective_solving_a_mystery_in_a_haunted_house-batch0-img7-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-22-30-target=An_alien_visiting_a_museum-batch0-img6-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-13_14-25-12-target=A_scientist_discovering_a_new_planet-batch0-img7-adv.png}
    \end{subfigure}%  
\end{minipage}

% Row 7


\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\textwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-02-58-target=A_dragon_playing_chess-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-02-26-target=A_robot_cooking_a_meal-batch0-img9-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-05-08-target=A_detective_solving_a_mystery_in_a_haunted_house-batch0-img7-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-04-35-target=An_alien_visiting_a_museum-batch0-img2-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-13_14-07-09-target=A_scientist_discovering_a_new_planet-batch0-img0-adv.png}
    \end{subfigure}%  
\end{minipage}

% \vspace{1em}
\caption{\textbf{Text inversion.} We show additional text inversion examples for \rclip (see Sec.~\ref{sec:text-inv}). Small initial step-size and large initial step-size are considered in the first and second rows respectively.
}
\label{fig:text-inv-app}
\end{figure*}

==> figures/text-inversion-full-workshop-2.tex <==
\begin{figure*}[h]
\centering
%\tiny
\footnotesize
% Row 1
%\textwidth=\columnwidth
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Mona Lisa by Leonardo da Vinci
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Guernica by\\Pablo Picasso
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        The Last Supper by Leonardo da Vinci
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        The Scream by Edvard Munch
    \end{minipage}%    
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Isaac Newton
    \end{minipage}% 
\end{minipage}


% eps=100, initial_stepsize=10
\vspace{0.5ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/mona_lisa.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/guernica.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/supper.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/scream.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_17-06-45-target=Isaac_Newton-batch0-img6-adv.png}
    \end{subfigure}% 
\end{minipage}

\vspace{0.5ex}
% row 2
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/mona-lisa.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/guernica.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/supper.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/scream.png}
    \end{subfigure}% 
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/newton.png}
    \end{subfigure}%
\end{minipage}

% row 3  
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{2mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Yoshua Bengio
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Boris Johnson
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        Elon Musk
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        The Terminator
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        An alien marketplace
    \end{minipage}%
\end{minipage}

\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_17-04-22-target=Yoshua_Bengio-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_17-01-54-target=Boris_Johnson-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_17-05-22-target=Elon_Musk-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_16-41-11-target=The_Terminator-batch0-img4-adv.png}
    \end{subfigure}%  
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_16-48-38-target=An_alien_marketplace-batch0-img1-adv.png}
    \end{subfigure}%
\end{minipage}

%  eps=200, initial_stepsize=none (i.e. 400)
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/bengio.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/johnson.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/musk.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/terminator.png}
    \end{subfigure}% 
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-06_15-09-20-target=An_alien_marketplace-batch0-img1-adv.png}
    \end{subfigure}%
\end{minipage}


% Row 5  
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{2mm}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        An octopus\\playing chess
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A penguin at\\the beach
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A dragon playing\\the piano
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A squirrel riding\\a skateboard
    \end{minipage}%
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        A werewolf howling\\at a full moon
    \end{minipage}%    
\end{minipage}

% Row 6  eps=200, initial_stepsize=none (i.e. 400)
\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_16-42-17-target=An_octopus_playing_chess-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_16-43-22-target=A_Penguin_at_the_beach-batch0-img5-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_16-48-07-target=A_dragon_playing_the_piano-batch0-img7-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_16-45-56-target=A_squirrel_riding_a_skateboard-batch0-img0-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/small-step/2024-03-06_16-47-35-target=A_werewolf_howling_at_a_full_moon-batch0-img5-adv.png}
    \end{subfigure}%  
\end{minipage}

% Row 7


\vspace{1ex}
\begin{minipage}[t]{.025\textwidth}
     \vspace{0pt}
\end{minipage}%
\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-06_15-03-06-target=An_octopus_playing_chess-batch0-img6-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-06_15-04-10-target=A_Penguin_at_the_beach-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-06_15-08-51-target=A_dragon_playing_the_piano-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-06_15-06-41-target=A_squirrel_riding_a_skateboard-batch0-img8-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{assets/text-inversion/big-step/2024-03-06_15-08-20-target=A_werewolf_howling_at_a_full_moon-batch0-img9-adv.png}
    \end{subfigure}%  
\end{minipage}

% \vspace{1em}
\caption{\textbf{Text inversion.} We show visual concepts encoded in \rclip by optimizing randomly initialized images to match the given text prompts in the embedding space. Small initial step-size and large initial step-size are considered in the first and second rows respectively. We are able to extract rich and meaningful visual concepts from \rclip.}
\label{fig:text-inv}
\end{figure*}

==> figures/text-inversion-full-workshop.tex <==
\begin{figure*}[h]
\centering
%\tiny
\footnotesize
% Row 1
%\figwidth=1.8\columnwidth
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
%\hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        Mona Lisa by Leonardo da Vinci
    \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        Guernica by\\Pablo Picasso
    \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        The Last Supper by Leonardo da Vinci
    \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        The Scream by\\Edvard Munch
    \end{minipage}%    
    % \begin{minipage}[t]{0.2\columnwidth}
    %     \centering
    %     Isaac Newton
    % \end{minipage}% 
\end{minipage}


% eps=100, initial_stepsize=10
%\vspace{0.5ex}
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
%\hspace{1ex}
% \begin{minipage}[t]{0.98\figwidth}
%     \vspace{0pt}
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/mona_lisa.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/guernica.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/supper.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/scream.png}
%     \end{subfigure}%  
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_17-06-45-target=Isaac_Newton-batch0-img6-adv.png}
%     \end{subfigure}% 
% \end{minipage}

\vspace{0.5ex}
% row 2
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
%\hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/mona-lisa.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/guernica.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/supper.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/scream.png}
    \end{subfigure}% 
    % \begin{subfigure}[t]{0.25\columnwidth}
    %     \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/newton.png}
    % \end{subfigure}%
\end{minipage}

% row 3  
\vspace{1ex}
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
% \hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{2mm}
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        Yoshua Bengio
    \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        Boris Johnson
    \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        Elon Musk
    \end{minipage}%
    % \begin{minipage}[t]{0.25\columnwidth}
    %     \centering
    %     The Terminator
    % \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        An alien marketplace
    \end{minipage}%
\end{minipage}

\vspace{.5ex}
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
% \hspace{1ex}
% \begin{minipage}[t]{0.98\figwidth}
%     \vspace{0pt}
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_17-04-22-target=Yoshua_Bengio-batch0-img0-adv.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_17-01-54-target=Boris_Johnson-batch0-img1-adv.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_17-05-22-target=Elon_Musk-batch0-img0-adv.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_16-41-11-target=The_Terminator-batch0-img4-adv.png}
%     \end{subfigure}%  
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_16-48-38-target=An_alien_marketplace-batch0-img1-adv.png}
%     \end{subfigure}%
% \end{minipage}

%  eps=200, initial_stepsize=none (i.e. 400)
%\vspace{1ex}
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
% \hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/bengio.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/johnson.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/musk.png}
    \end{subfigure}%
    % \begin{subfigure}[t]{0.2\columnwidth}
    %     \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/terminator.png}
    % \end{subfigure}% 
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/2024-03-06_15-09-20-target=An_alien_marketplace-batch0-img1-adv.png}
    \end{subfigure}%
\end{minipage}


% Row 5  
\vspace{1ex}
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
% \hspace{1ex}%
\begin{minipage}[t]{0.98\figwidth}
    \vspace{2mm}
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        An octopus\\playing chess
    \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        A penguin at\\the beach
    \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        A dragon playing\\the piano
    \end{minipage}%
    \begin{minipage}[t]{0.25\columnwidth}
        \centering
        A squirrel riding\\a skateboard
    \end{minipage}%
    % \begin{minipage}[t]{0.2\columnwidth}
    %     \centering
    %     A werewolf howling\\at a full moon
    % \end{minipage}%    
\end{minipage}

% Row 6  eps=200, initial_stepsize=none (i.e. 400)
% \vspace{1ex}
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
% \hspace{1ex}
% \begin{minipage}[t]{0.98\figwidth}
%     \vspace{0pt}
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_16-42-17-target=An_octopus_playing_chess-batch0-img1-adv.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_16-43-22-target=A_Penguin_at_the_beach-batch0-img5-adv.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_16-48-07-target=A_dragon_playing_the_piano-batch0-img7-adv.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_16-45-56-target=A_squirrel_riding_a_skateboard-batch0-img0-adv.png}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.2\columnwidth}
%         \includegraphics[width=\columnwidth]{assets/text-inversion/small-step/2024-03-06_16-47-35-target=A_werewolf_howling_at_a_full_moon-batch0-img5-adv.png}
%     \end{subfigure}%  
% \end{minipage}

% Row 7


\vspace{.5ex}
% \begin{minipage}[t]{.025\columnwidth}
%      \vspace{0pt}
% \end{minipage}%
% \hspace{1ex}
\begin{minipage}[t]{0.98\figwidth}
    \vspace{0pt}
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/2024-03-06_15-03-06-target=An_octopus_playing_chess-batch0-img6-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/2024-03-06_15-04-10-target=A_Penguin_at_the_beach-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/2024-03-06_15-08-51-target=A_dragon_playing_the_piano-batch0-img1-adv.png}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\columnwidth}
        \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/2024-03-06_15-06-41-target=A_squirrel_riding_a_skateboard-batch0-img8-adv.png}
    \end{subfigure}%
    % \begin{subfigure}[t]{0.2\columnwidth}
    %     \includegraphics[width=\columnwidth]{assets/text-inversion/big-step/2024-03-06_15-08-20-target=A_werewolf_howling_at_a_full_moon-batch0-img9-adv.png}
    % \end{subfigure}%  
\end{minipage}

% \vspace{1em}
\caption{\textbf{Text inversion.} We show visual concepts encoded in \rclip by optimizing randomly initialized images to match the given text prompts in the embedding space. %Small initial step-size and large initial step-size are considered in the first and second rows respectively.
We are able to extract rich and meaningful visual concepts from \rclip.
}
\label{fig:text-inv-short}
\end{figure*}

==> figures/text-inversion.tex <==
\begin{figure}[ht]
\centering

% Row 1
\begin{minipage}[t]{0.2\textwidth}
    \vspace{2em}
    This is the target text
\end{minipage}%
\hspace{2mm}%
\begin{minipage}[t]{0.75\textwidth}
\begin{subfigure}[t]{0.25\textwidth}
    \caption*{\vit}
    \includegraphics[width=\textwidth]{example-image-a}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \caption*{\vit \tecoa}
    \includegraphics[width=\textwidth]{example-image-a}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \caption*{\convnext}
    \includegraphics[width=\textwidth]{example-image-a}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \caption*{\convnext \tecoa}
    \includegraphics[width=\textwidth]{example-image-a}
\end{subfigure}%
\end{minipage}

%\vspace{0.5ex}
% Row 2
\begin{minipage}[t]{0.2\textwidth}
    \vspace{1em}
    This is another target text
\end{minipage}%
\hspace{2mm}%
\begin{minipage}[t]{0.75\textwidth}
\vspace{0pt}
\begin{subfigure}[t]{0.25\textwidth}
    \includegraphics[width=\textwidth]{example-image-b}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \includegraphics[width=\textwidth]{example-image-b}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \includegraphics[width=\textwidth]{example-image-b}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \includegraphics[width=\textwidth]{example-image-b}
\end{subfigure}%
\end{minipage}


\caption{Image generation}
\end{figure}
